RobotPerf: An Open-Source, Vendor-Agnostic, Benchmarking Suite for Evaluating Robotics Computing System Performance

We introduce RobotPerf, a vendor-agnostic benchmarking suite designed to evaluate robotics computing performance across a diverse range of hardware platforms using ROS 2 as its common baseline. The suite encompasses ROS 2 packages covering the full robotics pipeline and integrates two distinct benchmarking approaches: black-box testing, which measures performance by eliminating upper layers and replacing them with a test application, and grey-box testing, an application-specific measure that observes internal system states with minimal interference. Our benchmarking framework provides ready-to-use tools and is easily adaptable for the assessment of custom ROS 2 computational graphs. Drawing from the knowledge of leading robot architects and system architecture experts, RobotPerf establishes a standardized approach to robotics benchmarking. As an open-source initiative, RobotPerf remains committed to evolving with community input to advance the future of hardware-accelerated robotics.

==> tex/overview_results.tex <==
\includegraphics[width=\textwidth]{/tmp/report-color-coding.png}

\scriptsize
\renewcommand{\arraystretch}{2.5}

\begin{table}[h!]
\centering
\begin{tabular}{lcccc}
\toprule
 & \textbf{Perception} & \textbf{Localization} & \textbf{Control} & \textbf{Manipulation} \\
\midrule
\textbf{Latency (ms)} &
\includegraphics[width=0.2\textwidth]{/tmp/report-benchmarking-robotics-perception-latency-(ms)-multi-radar.png} &
\includegraphics[width=0.2\textwidth]{/tmp/report-benchmarking-robotics-localization-latency-(ms)-multi-radar.png} &
\includegraphics[width=0.2\textwidth]{/tmp/report-benchmarking-robotics-control-latency-(ms)-multi-radar.png} &
\includegraphics[width=0.2\textwidth]{/tmp/report-benchmarking-robotics-manipulation-latency-(ms)-multi-radar.png} \\
\midrule
\textbf{Throughput (FPS)} &
\includegraphics[width=0.2\textwidth]{/tmp/report-benchmarking-robotics-perception-throughput-(fps)-multi-radar.png} &
\includegraphics[width=0.2\textwidth]{/tmp/report-benchmarking-robotics-localization-throughput-(fps)-multi-radar.png} &
\includegraphics[width=0.2\textwidth]{/tmp/report-benchmarking-robotics-control-throughput-(fps)-multi-radar.png} & \\
\midrule
\textbf{Power (W)} &
\includegraphics[width=0.2\textwidth]{/tmp/report-benchmarking-robotics-perception-power-(w)-multi-radar.png} &
 &
\includegraphics[width=0.2\textwidth]{/tmp/report-benchmarking-robotics-control-power-(w)-multi-radar.png} &
\includegraphics[width=0.2\textwidth]{/tmp/report-benchmarking-robotics-manipulation-power-(w)-multi-radar.png} \\
\bottomrule
\end{tabular}
\end{table}
